TCFormer: Visual Recognition via Token Clustering Transformer

Transformers are widely used in computer vision areas and have achieved remarkable success. Most state-of-the-art approaches split images into regular grids and represent each grid region with a vision token. However, fixed token distribution disregards the semantic meaning of different image regions, resulting in sub-optimal performance. To address this issue, we propose the Token Clustering Transformer (TCFormer), which generates dynamic vision tokens based on semantic meaning. Our dynamic tokens possess two crucial characteristics: (1) Representing image regions with similar semantic meanings using the same vision token, even if those regions are not adjacent, and (2) concentrating on regions with valuable details and represent them using fine tokens. Through extensive experimentation across various applications, including image classification, human pose estimation, semantic segmentation, and object detection, we demonstrate the effectiveness of our TCFormer. The code and models for this work are available at https://github.com/zengwang430521/TCFormer.

==> sections/tcformer.tex <==


\begin{figure}[tb]
	\centering
	\includegraphics[width=0.48\textwidth]{image/transformer_block.pdf}
        \caption{
        Structure of the transformer blocks in TCFormer. 
        (a) To decrease computational complexity, a token reduction layer is employed to decrease the number of tokens. A depth-wise convolutional layer is included to extract local information.
        (b) The spatial token reduction module employs  a convolutional layer to reduce token number based on spatial relationship. 
        (c) The clustering  token reduction module reduces token number by merging tokens according to clustering results. 
        }
	\label{fig:block}
\end{figure}


\begin{figure*}[tb]
	\centering
	\includegraphics[width=0.9\textwidth]{image/ctm.pdf}
        \caption{
        Illustration of the dynamic vision token generation process. The Clustering-based Token Merge (CTM) module first groups the input tokens into several clusters and then merges the tokens in the same cluster into a single token via weighted feature averaging. In TCFormerV2, the input tokens are first divided into several parts based on their spatial location. The clustering algorithm is applied to each part independently. After the CTM module, the merged tokens and the original tokens are input into a transformer block for better feature aggregation.
        }
	\label{fig:ctm}
\end{figure*}


\section{Token Clustering Transformer} \label{sec:tcformer}
% The overall architecture of TCFormer is shown in Fig.~\ref{fig:arch}. TCFormer follows the popular pyramid structure and consists of 4 stages. Each stage is composed by several stacked transformer blocks. Between adjacent stages, a Clustering-based Token Merge (CTM) module is inserted to merge tokens dynamically, so that each stage processes tokens in different scales. The vision tokens in the first stage are initialized from a high resolution feature map by regarding each pixel in the feature as a token. After the last stage, a Multi-stage Token Aggregation (MTA) module aggregates multi-scale features in the format of vision tokens and outputs pyramid vision tokens for task-specific heads.
The overall architecture of TCFormer is shown in Fig.~\ref{fig:arch}. TCFormer adopts a popular pyramid structure, consisting of four stages. Each stage is composed by several stacked transformer blocks. A Clustering-based Token Merge (CTM) module is interspersed between adjacent stages to dynamically merge tokens and enable each stage to process tokens at varying scales. The vision tokens in the first stage are initialized from a high-resolution feature map, with each pixel in the feature map regarded as a token. After the final stage, a Multi-stage Token Aggregation (MTA) module integrates multi-scale features in the form of vision tokens and outputs a pyramid of vision tokens for task-specific processing.




\subsection{Transformer Block}
Fig.~\ref{fig:block} shows the structure of the transformer blocks in TCFormer. 
% As the token number in vision transformers is usually large, global attention process in traditional transformer block introduces unacceptable computational cost. To reduce the complexity, we add a token reduction module to reduce the token numbers before the attention process. After the attention process, we add a depth-wise convolutional layer to capture local information, which is proved beneficial by previous works~\cite{wu2021cvt,li2021localvit,yuan2021hrformer}.
Fig. 3 illustrates the structure of the transformer blocks in TCFormer. Due to the typically large number of tokens in vision transformers, global attention processes in traditional transformer blocks result in an unacceptable computational cost. To mitigate this problem, we incorporate a token reduction module before the attention process to reduce token numbers. After the attention process, we add a depth-wise convolutional layer to capture local information, as previously demonstrated by \cite{wu2021cvt,li2021localvit,yuan2021hrformer} to be beneficial.




% We propose two types of transformer blocks with different token reduction module: Spatial Reduction block (SR block) and Clustering Reduction block (CR block). As shown in Fig.~\ref{fig:block}(b), spatial token reduction module transfers vision tokens to feature map first and then shrinks the feature map resolution with a convolutional layer. The down-sampled feature map is flattened as the key and value tokens with the reduced token number. As shown in Fig.~\ref{fig:block}(c), clustering token reduction module reduces the token number by merging the tokens according to the clustering results. Compared with SR block, CR block is more efficient. As CR block requires the clustering results, we only apply it in the Multi-stage Token feature Aggregation (MTA) module. Specifically, we apply CR blocks in the MTA module of TCFormerV2 and use SR blocks in the other modules.
%
We propose two types of transformer blocks with different token reduction modules: the Spatial Reduction(SR) block and the Clustering Reduction(CR) block. The SR block (as shown in Fig. 3(b)) transfers vision tokens to a feature map, then shrinks the feature map resolution with a convolutional layer. The down-sampled feature map is then flattened to form the key and value tokens with a reduced number of tokens. On the other hand, the CR block (as shown in Fig. 3(c)) reduces the token number by merging tokens based on the clustering results. Compared to the SR block, the CR block is more efficient. However, since the CR block requires the clustering results, it is only applied in the Multi-stage Token Aggregation (MTA) module. Specifically, we use CR blocks in the MTA module of TCFormerV2 and SR blocks in all other modules.





\subsection{Clustering-based Token Merge (CTM) Module}
% As shown in Fig.~\ref{fig:ctm}, our Clustering-based Token Merge (CTM) module is composed of the token clustering and merging process. Given the vision tokens in the previous stage, CTM module first groups vision tokens into a certain clusters by applying a clustering algorithm to the token features, and then merges the token in the same cluster to get new vision tokens for the next stage.
%
As shown in Fig.~\ref{fig:ctm}, the Clustering-based Token Merge (CTM) module of our TCFormer is comprised of a token clustering and merging process. Given the vision tokens from the prior stage, the CTM module first groups the tokens into clusters through the application of a clustering algorithm to the token features, and then merges the tokens within the same cluster to generate new vision tokens for the subsequent stage.


\textbf{Token Clustering.}
% For token clustering process, we apply a variant of the k-nearest neighbor based density peaks clustering algorithm (DPC-kNN)~\cite{du2016study} for its simplicity and parallelism. 
% Given a set of vision tokens $X$, for each token, we first calculate the distance between it and other tokens and then estimate the local density $\rho$ from the distance between its k-nearest neighbors:
%
For the token clustering process, we utilize a variation of the density peaks clustering algorithm based on k-nearest neighbors (DPC-kNN)~\cite{du2016study}, due to its simplicity and parallelization capabilities.
Given a set of vision tokens $X$, we first calculate the distance between each token and the other tokens. Then, we estimate the local density $\rho$ from the distances between the token and its k-nearest neighbors:
%
\begin{equation}
\rho_{i}=\exp \left(-\frac{1}{k} \sum_{x_{j} \in \mathrm{kNN}\left({x}_{i}\right)} 
\left\|x_i-x_j\right\|_{2}^{2},
\right),
\label{eq:rho}
\end{equation}
where $\mathrm{kNN}\left({x}_{i}\right)$ denotes the k-nearest neighbors of a token $i$. $x_i$ and $x_j$ are their corresponding token features.

Then for each token, we collect the distance between it and the tokens with higher local density, and use the minimal distance as the distance indicator. Tokens with large distance indicator tends to be local density peaks and are considered suitable candidates of clustering centers. For the token with highest local density, we set the maximum distance between it and other tokens as its distance indicator to make sure that it has the largest distance indicator.
\begin{equation}
\delta_{i}=\left\{\begin{array}{l}
\min _{j: \rho_{j}>\rho_{i}} \left\|x_i-x_j\right\|_{2}, \text { if } \exists j \text { s.t. } \rho_{j}>\rho_{i} \\
\max _{j} \left\|x_i-x_j\right\|_{2}, \text { otherwise }
\end{array}\right.
\label{eq:delta}
\end{equation}
where $\delta_{i}$ denotes the distance indicator and $\rho_{i}$ denotes the local density.

% Finally, we multiply the local density with the distance indicator to get the score of each token as $\rho_i \times \delta_i$. Higher scores mean higher potential to be cluster centers. We selects the tokens with the highest scores as clustering centers and assigns other tokens to their nearest center. 
Finally, we determine the score of each token by multiplying its local density by its distance indicator, resulting in $\rho_i \times \delta_i$. Tokens with higher scores possess a greater likelihood of being cluster centers. The tokens with the highest scores are then selected as clustering centers, and the remaining tokens are allocated to the nearest center.

\textbf{Token Merging}
% Token merging process aims to generate a new vision token for each cluster, which is representative of the cluster. An intuitive method is to average the token features in the cluster directly. However, simple averaging ignores the difference of token importance. Inspired by previous works~\cite{rao2021dynamicvit,meng2022adavit,wang2021pnp}, we predict importance score $P$ from the token features to indicate the importance of tokens and guide the feature averaging with the predicted importance scores:
%
The token merging process endeavors to produce a single representative token for each cluster. A straightforward approach would be to simply average the token features within the cluster. However, this ignores the varying significance of each token. Drawing inspiration from prior works~\cite{rao2021dynamicvit,meng2022adavit,wang2021pnp}, we predict the importance score $P$ of each token based on its features to reflect its significance and guide the averaging of token features using the predicted importance scores:
%
\begin{equation}
y_{i}=\frac {\sum_{j \in C_i} e^{p_j} x_j}
            {\sum_{j \in C_i} e^{p_j}} ,
\label{eq:average}
\end{equation}
where $C_i$ means the set of the $i$-th cluster, $x_j$ and $p_j$ are the original token feature and the corresponding importance score respectively. $y_i$ is the features of the merged token.

% As shown in Fig.~\ref{fig:ctm}, the original tokens and merged tokens are fed into the next transformer block, where the merged tokens serve as queries and the original tokens serve as keys and values. The transformer block aims to transfer features from the original tokens to the merged tokens and the importance score $P$ is involved in the attention process to guide the feature transfer process.
%
As depicted in Fig.~\ref{fig:ctm}, the original tokens and the merged tokens are input into the subsequent transformer block, with the merged tokens functioning as queries and the original tokens serving as keys and values. The transformer block aims to transfer features from the original tokens to the merged tokens, with the importance score $P$ incorporated into the attention mechanism to steer the feature transfer process.
%
\begin{equation}
\operatorname{Attention}(Q, K, V)=\operatorname{softmax}\left(\frac{Q K^{T}}{\sqrt{d_{k}}}+P\right) V,
\label{eq:attn}
\end{equation}
where $d_k$ is the channel dimension of the queries. 
% We omit the multi-head setting and the spatial reduction layer here for clarity. Introducing the token importance score into the feature averaging and attention process enables the important vision tokens to contribute more to the output dynamic tokens.
%
For clarity, we omit the multi-head setting and the spatial reduction layer. By incorporating the token importance score into both the feature averaging and attention processes, we ensure that the crucial visual tokens have a greater impact on the output dynamic tokens.


\begin{figure}[tb]
	\centering
	\includegraphics[width=0.48\textwidth]{image/mta_token.pdf}
        \caption{
        A typical example of the dynamic tokens produced by TCFormer. The input image is depicted in (a), and the dynamic tokens are presented in (b). The dynamic tokens can be converted into a high-resolution feature map (c), which retains the details but leads to large computational complexity, or a low-resolution feature map (d), which sacrifices the detailed information in the dynamic tokens.
        }
	\label{fig:mta_token}
\end{figure}

\begin{figure}[tb]
	\centering
	\includegraphics[width=0.48\textwidth]{image/mta.pdf}
        \caption{
        Illustration of the Multi-Stage Token Aggregation (MTA) Module. (a) During the token upsampling process, we use the recorded token relationship to copy the merged token features to the corresponding upsampled tokens. (b) The MTA module starts from the final stage and progressively accumulates features through sequential upsampling procedures and transformer blocks. The tokens at every stage are transformed to create a feature map pyramid for further processing.
        }
	\label{fig:mta}
\end{figure}


\textbf{Local CTM module}
% As mentioned above, the original CTM module involves the calculation of the distance between any token pairs, which brings huge complexity in early stages because of the large token numbers. Fortunately, we observe that vision tokens tends to merge with the neighboring tokens in early stages. So we propose a local token clustering method to reduce the complexity. We first split the input tokens into several parts according the the spatial location and then apply the clustering algorithm to each part separately. By this mean, the local CTM module only needs to calculate the distance between local token pairs but get similar results as the global CTM module. 
%
As previously noted, the original CTM module requires the computation of the distance between every token pair, leading to high complexity in the early stages due to the substantial number of tokens. However, we observe that vision tokens tend to merge with their adjacent tokens in the early stages. To mitigate this complexity, we propose a local token clustering method. We divide the input tokens into several parts based on their spatial location and apply the clustering algorithm to each part individually. In this manner, the local CTM module only needs to calculate the distance between local token pairs, but yields results comparable to the global CTM module.



% We apply local CTM module in TCFormerV2. We split tokens to more parts in early stage and shrink the part number in later stages. Specifically, for the tokens in stage 1 and stage 2, we split them into 16 and 4 parts respectively. While for the tokens in stage 3, we use the original global CTM module.
%
We employ the local CTM module in TCFormerV2, gradually reducing the number of parts as the stages progress. Specifically, in stage 1 and stage 2, the tokens are divided into 16 and 4 parts, respectively. In stage 3, the original global CTM module is used.













\subsection{Multi-stage Token Aggregation (MTA) Module}
\label{sec:tcformer:mta}
% Multi-scale feature aggregation is proved beneficial for various tasks~\cite{sun2019deep,lin2017feature,zhu2020deformable}. Previous vision transformers~\cite{wang2021pyramid,liu2021swin,yuan2021hrformer} transfer vision tokens to feature map and aggregate multi-scale features with traditional convolutional neural networks. However, it's not suitable for our dynamic vision tokens.
%
The integration of multi-scale features has been demonstrated to be beneficial for various tasks~\cite{sun2019deep,lin2017feature,zhu2020deformable}. Previous vision transformers~\cite{wang2021pyramid,liu2021swin,yuan2021hrformer} transform vision tokens into feature maps and aggregate multi-scale features using conventional convolutional neural networks. However, this approach is not suitable for our dynamic vision tokens.


% As shown in Fig.~\ref{fig:mta_token}, TCFormer allocates fine tokens for important image regions with detail information. Transforming vision tokens to low resolution feature map as previous works~\cite{sun2019deep,lin2017feature,zhu2020deformable} leads to the loss of details. In contrast, transforming our dynamic vision tokens to high resolution feature map keeps the details, but involves unacceptable complexity and memory cost. Instead of transform vision tokens to feature maps, we propose a transformer based Multi-stage Token Aggregation (MTA) module to aggregate features in the format of tokens.
%
As shown in Fig.~\ref{fig:mta_token}, TCFormer assigns fine tokens to image regions that contain intricate details. Transforming our dynamic tokens into low-resolution feature maps, as previous works~\cite{sun2019deep,lin2017feature,zhu2020deformable} have done, results in a loss of detail. In contrast, transforming the tokens into high-resolution feature maps retains the details but incurs unacceptable complexity and memory overhead. Rather than transforming vision tokens into feature maps, we propose a transformer-based Multi-stage Token Aggregation (MTA) module that aggregates features in the form of tokens.


% We first define the upsampling process of our dynamic vision token. As shown in Fig.~\ref{fig:mta}(a), in CTM modules, we group tokens to multiple clusters and merge the tokens in the same cluster to a single token. The clustering results are recorded for token upsampling process, where we copy the features from the merged tokens to the corresponding upsampled tokens following the recorded clustering results.
%
We first establish the definition of our dynamic vision token upsampling process. As shown in Fig.~\ref{fig:mta}(a), in the CTM modules, we group tokens into multiple clusters and consolidate the tokens within each cluster into a single token. The clustering results are recorded for the token upsampling process, in which the features from the merged tokens are replicated to the corresponding upsampled tokens based on the recorded clustering results.




% Following FPN~\cite{lin2017feature}, MTA module aggregates features from deep stages to shadow stages gradually. As shown in Fig.~\ref{fig:mta}(b), the vision tokens in the last stage are regarded as the initial tokens. At every step, MTA module first upsamples the vision tokens, so that the upsampled tokens are in the same distribution as the tokens in the previous stage. Then MTA module adds the token features in the previous stage to the upsampled tokens and fed the results to a transformer block. Above step is executed repeatedly until token features from all stages are aggregated. Finally, the tokens in every step are transformed to pyramid feature maps for further processing.
%
Following FPN~\cite{lin2017feature}, the MTA module gradually aggregates features from deeper stages to shallower stages. As shown in Fig.~\ref{fig:mta}(b), the visual tokens in the final stage are considered as the starting tokens. At each step, the MTA module first upsamples the visual tokens so that the upsampled tokens have the same distribution as the tokens in the preceding stage. The MTA module then adds the token features from the preceding stage to the upsampled tokens and inputs the results into a transformer block. This process is repeated until features from all stages have been aggregated. Finally, the tokens at each step are transformed into pyramid feature maps for further processing.
%
% By aggregating features in the format of vision tokens, MTA module reserves the details in every stage and avoids processing the high resolution feature maps. It achieves the balance between performance and efficiency.
%
By aggregating features in the form of vision tokens, the MTA module preserves the details at each stage and sidesteps the processing of high-resolution feature maps, striking a balance between performance and efficiency.

We propose two versions of the MTA module with differences in the transformer blocks they utilize. The first version, called SR-MTA, utilizes SR blocks and is implemented in TCFormerV1. The second version, called CR-MTA, utilizes CR blocks and is utilized in TCFormerV2.



% In TCFomerV1~\cite{zeng2022not}, MTA block transforms the final vision tokens to high resolution feature map for further processing. While in TCFormerV2, MTA block combines the vision tokens in every step to form a token pyramid for the following process.







\subsection{Comparison of TCFormer Variants}
We develop two types of TCFormer models: TCFormerV1 and TCFormerV2. The comparison between them is presented below.
% A comparison between them is presented in Table~\ref{tab:variants}.

\noindent\textbf{TCFormerV1.} 
TCFormerV1 utilizes global CTM modules to generate dynamic tokens and a SR-MTA module to aggregate token features. This model is used in the preliminary paper~\cite{zeng2022not}.

\noindent\textbf{TCFormerV2.} 
TCFormerV2 is an improvement version over TCFormerV1, accomplished by introducing local CTM modules and CR-MTA module. Compared to TCFormerV1, TCFormerV2 is more efficient and can learn object relationships more effectively.

In this paper, we will show the results of applying both TCFormerV1 and TCFormerV2 to image classification, human pose estimation, and semantic segmentation. Regarding object detection, TCFormerV1 brings unacceptable complexity, so we only apply TCFormerV2 to this task.


% \begin{table}[t]
%     \centering
%     \caption{Comparisons of TCFormerV1 and TCFormerV2.}
%     \label{tab:variants}
%     \scalebox{0.95}{
%     \begin{tabular}{l|c|c}
%     \Thline
%     \renewcommand{\arraystretch}{0.1}
%     Variants & CTM module & MTA module \\
%     \Thline
%     TCFormerV1 & Global CTM & SR-MTA \\
%     TCFormerV2 & Local CTM & CR-MTA \\
%     \Thline
% \end{tabular}}
% \end{table}
